Architecture-Aware, High Performance Transaction for Persistent Memory

Byte-addressable non-volatile main memory (NVM) demands transactional mechanisms to access and manipulate data on NVM atomically. Those transaction mechanisms often employ a logging mechanism (undo logging or redo logging). However, the logging mechanisms can bring large runtime overhead (8%-49% in our evaluation), and 41%-78% of the overhead attributes to the frequent cache-line flushing. Such large overhead significantly diminishes the performance benefits offered by NVM. In this paper, we introduce a new method to reduce the overhead of cache-line flushing for logging-based transactions. Different from the traditional method that works at the program level and leverages program semantics to reduce the logging overhead, we introduce architecture awareness. In particular, we do not flush certain cache blocks, as long as they are estimated to be eliminated out of the cache because of the hardware caching mechanism (e.g., the cache replacement algorithm). Furthermore, we coalesce those cache blocks with low dirtiness to improve the efficiency of cache-line flushing. We implement an architecture-aware, high performance transaction runtime system for persistent memory, Archapt. Our results show that comparing with an undo logging (PMDK) and a redo logging (Mnemosyne), Archapt reduces cache-line flushing by 66% and improves system throughput by 19% on average (42% at most). Our crash tests with four hardware caching policies show that Archapt provides a strong guarantee on crash consistency.

==> text/design_old.tex <==
\section{Design}















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Undo logging and redo logging are two well known transactional persistence techniques. Though promising, they both have oblivious performance bottlenecks. In this section, we first analyze the benefits and limitations of Undo logging and Redo logging on persistent memory, then we introduce a new programming model based persistent memory transaction technique called Ru logging. Taken the non-volatility and good performance of emerging persistent memory, Ru logging is an optimized persistent technique to overcome drawbacks of Undo logging and redo logging.

\subsection{Redo logging and Undo logging}
\textbf{Undo}
Within an undo logging based transaction, a log of unmodified data is created before every data writing operation, and such log copy will be persisted immediately. After that, in-place data updating happens on original data copy and updated data needs to persist as well. Once one transaction fails, any modifications are ignored and are rolled back to the latest version data in the log. Guarantee the writing order, on the one hand, is costly; but on the one hand, it makes the read operation lightweight without extra tracking overhead (e.g. read-after-write access).

\textbf{Redo}
Within a redo logging based transaction, a log will be created and all updated data is appended to such log. Different from Undo logging, redo logging does not require the ordering constraints on write operations. We only need to persist all the write operations before the transaction committed. All updated data on the log will be applied to original data copy when the transaction committed. If a failure happens during the transaction, the redo log will be discarded. Async persistence of write operations reduce the write ordering constraint overhead. However, it brings the additional overhead to the read operation because of read-after-write access challenge. All the read operations need to traverse the entire log to find the newest value since the latest version data only stores in the log.  


In the Table~\ref{tab:summary_undo_redo}, we summarize the benefits and limitations of undo logging and redo logging. Motivated by those features, we propose the ru logging technique that adopted to the persistent memory.   

\begin{table}
 \small
        \begin{center}
            \caption{Summary of Undo and Redo log.}
   %    \vspace{-10pt}
          \label{tab:summary_undo_redo}
\begin{tabular}{|p{1.8 cm}|p{1.8 cm}|p{1.8 cm}|p{1.8 cm}|}
       \hline
\multicolumn{2}{c|}{\textbf{Undo}} & \multicolumn{2}{c|}{\textbf{Redo}} \\ 
       \hline 
Benefits   & limitation   & Benefits  & limitation    \\ \hline \hline
XXX  & 1. need to persist every write  & XXX & 1. expensive log traverse to find the latest data  \newline 2. Overhead to apply all modified data to original version  \\\hline
%195.0 &248.3 &263.3  &257.6  \\\hline
%49.9\% & 3.9\% & 4.6\% & 5.5\%      \\ \hline
%$ 4.7 \times 10^3 $ & 0.008 & 0.02 & 0.02       \\ \hline
\end{tabular}
\end{center}
% \vspace{-20pt}
\end{table}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}
\lstdefinestyle{style1}{
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\footnotesize,
    frame=single,
%    breakatwhitespace=false,         
%    breaklines=true,                 
%    captionpos=b,                    
%    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt, 
%    showspaces=false,                
%    showstringspaces=false,
    %showtabs=false,                  
    %tabsize=2
	escapeinside={(*@}{@*)},
}
\lstset{style=style1}

\begin{figure}[!htb]
\centering
%\vspace{-10pt}
\begin{tabular}{c p{0.1cm} c}

\begin{lstlisting}[language=c, 
xleftmargin=.02\textwidth, xrightmargin=0.01\textwidth]
class bitMap{

}

class dataNode{
	int key;
    double value;
}

class ruTransaction{
	dataNode *dataRecord[2];   
    // 0 -> working version; 1 -> persistent version\
    bitMap writeStatus;
    int recordSize;
}

\end{lstlisting}
\end{tabular}
%\end{center}
%\vspace{-10pt}
\caption{Key data structure of ru logging.}
\label{fig:ru_data_struture}
%\vspace{-20pt}
\end{figure}

\subsection{Ru logging}
The key idea of ru logging is aim to remove data copying of logging by leveraging application-inherent memory write operations to create a new version of the target data record of each transaction. Figure~\ref{fig:ru_data_struture} shows the data structure of ru logging.

In details, ru logging allocates an extra copy of the logging data record when such record is created at the first time. Thus, there are two versions of the data record. One is working version (dataReocrd[0] in Figure~\ref{fig:ru_data_struture}), the other is persistence version (dataRecord[1] in Figure~\ref{fig:ru_data_struture}). Two versions of the data record are involved in each transaction, but memory write operations only happen to working version of the data record, the persistent version record remains unchanged until the next transaction. At the end of each transaction, the working version 
is flushed out of the cache and becomes persistent in persistent memory. 
This version will not be changed in the next transaction, and 
becomes the persistent version since then.
The previous persistent version becomes the working version,
and is updated by the memory write operations of the application.
Two versions alternate roles across transaction, with one version being persistent and the other being updated. Hence, we ensure that there is always a persistent version in persistent memory for restart. 

\textbf{Version management}
For each transaction, ru logging uses dual versions of target data record to instead of multiple version. The reason that undo logging and redo logging adopt multiple versions in a single transaction is traditional storage (e.g. hard drive and SSD) has a relative slow performance. Frequent data reload from storage into memory can be a bottleneck. However, taken the memory-class speed of persistent memory, ru logging can quickly switch the record version without data reload overhead in persistent memory. Therefore, it is very efficient to backtrack the log record since ru logging only has two versions. Memory footprint is also reduced by using dual version mechanism in ru logging. 

\textbf{Load instrumentation}
However, similar to redo logging, read-after-write access is a challenge for ru logging. It is because the modified new value only appears in the working version. To overcome this problem, redo logging traverse the whole log to find the latest value for every read operation. It definitely brings the significant overhead. To minimize such overhead, ru logging maintains a bitmap as an indicator to shows the write status (0 means no write on such element yet in the current transaction; 1 means such data element has been updated in current transaction) each data element of data record in the transaction. For each read operation, we only need to check the corresponding bitmap to determine the data is read from persistent version or working version.

\textbf{Persistent barrier}

\textbf{Log-record persistence}
Taken the advantage of the in-place update, ru logging does not need any data copy from working version to persistent version. At the end of the transaction, ru logging will flush the processor cache and write back the data from the cache to memory. Then ru logging switches the pointer of working version record and persistent version record. To optimize the cache flushing, we adopt the async cache flushing mechanism to improve the performance which described the Section ~\ref{} (TODO: helper thread + working thread idling time + full cache flush[cache locality].

\textbf{Apply the update to data record}
Since ru logging is the in-place update, applying the new update to the data record is easy. Different from the redo logging that needs copy the modified data from the log to the working data, ru logging just switch the role of two versions of the data record at the end of each transaction.

\textbf{Resize the record}
Flexible extend or shrink the log size is critical to the performance of logging mechanism. Ru logging can efficiently implement it by comparing the size of working version of record to the persistent version of record at the begin of the transaction. If their sizes are same, then the current transaction can simply update on working version of the record; if their sizes are different, a new working version will be allocated in persistent version record size. 

\textbf{Crash recovery}
If there is failure happens in the transaction, ru logging will ignore the modification on working version and restart the persistent version.

Overall, ru logging has following advantages compares with undo logging and redo logging.
%\begin{comment}
%(1) version management (multiple version or not) and why the version management is designed like that.

%(2) load instrumentation

%(3) the persistent barrier (how many of them and why)

%(4) log-record persistence (how and why)

%(5)  how to apply the update (e.g., redo-log is re-applied to the original data copy at the end of the transaction.)

%(6) how to extend the data

%(7) crash recovery
%\end{comment}

%\begin{comment}
%\definecolor{codegreen}{rgb}{0,0.6,0}
%\definecolor{codegray}{rgb}{0.5,0.5,0.5}
%\definecolor{codepurple}{rgb}{0.58,0,0.82}
%\definecolor{backcolour}{rgb}{0.95,0.95,0.92}
%\lstdefinestyle{style1}{
%    commentstyle=\color{codegreen},
%    keywordstyle=\color{magenta},
%    numberstyle=\tiny\color{codegray},
%    stringstyle=\color{codepurple},
%    basicstyle=\footnotesize,
%    frame=single,
%    breakatwhitespace=false,         
%    breaklines=true,                 
%    captionpos=b,                    
%    keepspaces=true,                 
%    numbers=left,                    
%    numbersep=5pt, 
%    showspaces=false,                
%    showstringspaces=false,
    %showtabs=false,                  
    %tabsize=2
	%escapeinside={(*@}{@*)},
%}
%\lstset{style=style1}

%\begin{figure}[!htb]
%\centering
%\vspace{-10pt}
%\begin{lstlisting}[language=c, 
%xleftmargin=.02\textwidth, xrightmargin=0.01\textwidth]
%#pragma omp task \
%    in(([realN]oldPanel)[1;BS][1;BS] ...) out (...)      
%void jacobi(long realN, long BS, \
%        double newPanel[realN][realN], \
%        double oldPanel[realN][realN]) {
%  for (int i=1; i <= BS; i++) {
%    for (int j=1; j <= BS; j++) {%
	  %newPanel[i][j] = 0.25 * (oldPanel[i-1][j] \
       %   + oldPanel[i+1][j] + oldPanel[i][j-1] \
    %      + oldPanel[i][j+1]);
%} } }

%void main(){
%...
%#pragma omp taskwait
%for (int iters=0; iters<L; iters++) {
%  int currentPanel = (iters + 1) % 2;
%  int lastPanel = iters % 2;	
%  for (long i=BS; i <= N; i+=BS) {
%    for (long j=BS; j <= N; j+=BS) {
%      jacobi(realN, BS, \
%            (m_t) &A[currentPanel][i-1][j-1], \
%            (m_t) &A[lastPanel][i-1][j-1] );           
%} } }
%#pragma omp taskwait
%...
%}
%\end{lstlisting}
%\end{center}
%\vspace{-10pt}
%\caption{Code snippet from a task parallel benchmark (heat).}
%\label{fig:task_code_example}
%\vspace{-20pt}
%\end{figure}
%\end{comment}






==> text/use_case.tex <==
%\section{Use Cases}
\section{Applying \name{} to Undo and Redo Logging}
\label{sec:use_cases}

Undo log-based and redo log-based transactions are two of the most common mechanisms to build persistent transactions on persistent memory. %%They are widely adopted in the current systems~\cite{Oracle,reid2012instant}. 
%We describe how Archa is applied to them in this section.

\begin{comment}
\begin{figure}
\includegraphics[width=0.48\textwidth, height=0.2\textheight] {figures/undo_redo_edit.pdf}
\caption{An example of the undo log-based and redo log-based
transactions. The undo log-based transaction needs two sync cache line flushing(s); The redo log-based transaction needs two async cache line flushing(s), one store fence, and one sync cache line flushing.}
\label{fig:undo_redo}
\end{figure}
\end{comment}

%\textbf{Undo Log-based Persistent Transactions.}
With undo-logging, %When the transaction writes to a persistent object, 
system first copies the original data of the persistent object into a newly allocated log and triggers synchronous cache-line flushing to persist the log record. Then committing the update on the persistent object in-place and flushing the cache-lines correspondingly. %. Once the data copy finishes, the undo log mechanism triggers synchronous cache-line flushing to persist the log record. The log record must be persisted before the object is updated in place. Meanwhile, every write happens on the persistent objects needs to be persisted. %Figure~\ref{fig:undo_redo}.a shows the pseudo code of the undo log mechanism. 


%%A typical implementation of the undo log uses a chunked list to organize the log records. The new log record is appended to the end of the list. This indicates that whenever a new log record is added, the tail pointer of the chunked list needs to be updated and immediately persisted using a synchronous cache-line flushing and a persistent barrier. An undo log transaction is committed by ensuring that all transactional writes are persisted (using one persist barrier). %and a commit record is appended to the transaction's undo log.  

%Finally, we commit the transaction and make the modified data persistent. We describe the pseudocode of undo log-based transaction in the figure~\ref{fig:undo_redo} (a).



%%Figure~\ref{fig:undo_redo}.a shows the pseudo code of the undo log mechanism. The figure shows a transaction, and there is an update to a persistent object $A$ in the transaction. With the undo log, there are two synchronous cache-line flushing and two persistent barriers (one to persist the log record and the other to persist the tail pointer of the chunked list), and there is also a cache-line flushing and a barrier to persist the most recent update when the transaction is committed. With the undo log, the update to the data happens in place. Hence a read operation can easily find the most recent update. However, multiple cache-line flushing and barriers are expensive and largely impact performance.

%Within an undo log-based persistent transaction, we need to copy the old version data to a new allocated undo log location on persistent memory before each data update operation. Once the data copy complete, one synchronous cache write-back operation is triggered immediately. The synchronous cache write-back operation means a $clwb$ instruction with a $sfence$ instruction. After that, we modify the old version data in place immediately. Typically, we use a chunked list to organize the undo log. Therefore, we need to update the tail pointer of the chunked list after every new undo log record inserted and then write-back the data for the tail pointer synchronously. Synchronous cache write-back operation ensures that the log data reach the persistent memory immediately after they are issued. Finally, we commit the transaction and make the modified data persistent. We describe the pseudocode of undo log-based transaction in the figure~\ref{fig:undo_redo} (a).Suppose we have one append one object A in a transaction, we need to issue two synchronous cache write-back operations on log writing, and one synchronous cache write-back on data while we commit the transaction. For two synchronous cache write-back operations on the log, one is to persist the new log record; the other is to persist tail pointer of the log list. Undo log-based approach always read and update the most recent data directly. But the synchronous cache write-back is an expensive operation and can largely impact the performance.

%\begin{comment}
%\begin{figure}
%\begin{tcolorbox}
%\begin{verbatim}
%TX_BEGIN(){
%		copy: data(A) -> log(A);
%	    persist: log(A);
%	    update: log_pointer;
%	    persist: log_pointer;
%		update: data(A);
%		…… (N-1 writes)
%} TX_END
%\end{verbatim}
%\end{tcolorbox}
%\caption{An example of undo log-based transaction and redo log-based transaction.}
%\label{fig:undo_code}
%\end{figure}
%\end{comment}

\begin{comment}
\begin{table}
        \begin{center}
       % \vspace{-10pt}
        \label{tab:api}
       % \scriptsize
               \caption{Comparison of Undo, Redo and Archa in terms of persistent overhead. Suppose there are $N$ objects updated in a transaction. The reported values for Archa is the optimal number. Depending on how the objects are reused within and across transactions, the persistent overhead of Archa will vary, but always be smaller than undo and redo logging. }
        \begin{tabular}{|p{2.5cm}|p{2.5cm}|p{2.5cm}|}
        \hline
        \textbf{Log Techniques}     & Number of Cache-line flushing   & Number of barriers                              \\ \hline \hline
        Undo      & 3N & 3N    \\\hline
        Redo      & 3N & N+1            \\ \hline
        Archa       & 0 & 0                 \\ \hline
        \end{tabular}
        \end{center}
      %  \vspace{-13pt}
\end{table}
\end{comment}


%\textbf{Redo Log-based Persistent Transactions.}
%Different from the undo log mechanism that update data in place, the redo log mechanism appends all updates to the newly allocated redo log. Each new log record of the redo log does not need to be durable until all log records for that transcation have been writen. cache line flushing triggered after the log record appended wrtite but does not need to be durable on NVM at the time of the write. RedoThe store barrier is before the  An asynchronous cache write-back is acceptable but must be completed right before we commit the transaction. After we commit the transaction, we need to re-apply (copy) the new redo log record data back to original application data area and make it persitent as well. 
%Different from the undo log mechanism that update data in place, the redo log mechanism appends all updates to the newly allocated log record. Each new log record does not need to be durable at the time of write. Redo log only guarantees all log records are persisted before any log content update to data. Hence, transaction abort causes the system to discard the entire redo log. 
%Different from the undo log mechanism that updates persistent objects in-place, 
With redo-logging, system first produces a log record containing the new value of the persistent object and flushes the cache lines for the log record asynchronously. Once the asynchronous  cache-line flushing for log record has been completed, the system applies the new content of log record to the persistent object and flushes cache-lines for the persistent object. %Figure~\ref{fig:undo_redo}.b shows the pseudo code of the redo log mechanism for the same example as in Figure~\ref{fig:undo_redo}.a. 

%%Similar to the undo log, the redo log is implemented as a chunked list. When a new log record is added, the redo log mechanism must update the tail pointer of the list and persist the update. Also, when committing a transaction, the redo log mechanism must finish flushing redo log records with a persistent barrier, applies redo logs to modified objects, and issue another barrier. 
%%\textcolor{blue}{(double-check if the above paragraph is correct)}
%In total, the redo log mechanism requires at least two persistent barriers (besides the two barriers discussed above, more barriers may be needed to bookkeep the transaction state as either COMMITTED or IDLE).

\begin{table}
        \begin{center}
       % \vspace{-10pt}
        \label{tab:comparison_undo_redo_archa}
       % \scriptsize
               \caption{Comparison of Undo, Redo and Archa in terms of persistent overhead. Suppose there are $N$ objects updated in a transaction. The reported values for Archa is the optimal number. Depending on how the objects are reused within and across transactions, the persistent overhead of Archa will vary, but always be smaller than undo and redo logging. }
        \begin{tabular}{|p{2.5cm}|p{2.3cm}|p{2.3cm}|}
        \hline
        \textbf{Log Techniques}     & Number of Cache-line flushing   & Number of barriers                              \\ \hline \hline
        Undo      & 2N & 2N    \\\hline
        Redo      & 2N & N+1            \\ \hline
        Undo-\name{}       & N & N                 \\ \hline
        Redo-\name{}       & N & 1                 \\ \hline
        \end{tabular}
        \end{center}
      %  \vspace{-13pt}
\end{table}

Though undo logging and redo logging are different, applying \name{} with them remains same. \name{} does not skip cache-line flushing for log record because of the transaction semantics. Hence, \name{} does not modify any logging procedure. \name{} skips cache-line flushing for persistent objects. Any cache-line flushing action for writing the persistent object is pending and is to be determined by reuse information of the persistent object based on LRU queue. The write operation on persistent object can be committing the updates in-place on the persistent object in undo logging and also can be applying the new content of log record on the persistent object in redo logging.  

%%We skip the cache-line flushing for persistent objects. The cache-line flushing can be triggered due to the data reuse within transaction and due to the data reuse of previous update. 



%Similar to the undo log, the redo log is managed as a chunked list. The tail pointer update of the chunked list is required after each new log record inserted. However, the store barrier after each write is waived due to the redo log reduces the constraints on writes to NVM. The additional overhead of the redo log is all the read operations in a transaction has to consult the log for the latest value.

%%Figure~\ref{fig:undo_redo}.b shows the pseudo code of the redo log mechanism for the same example as in Figure~\ref{fig:undo_redo}.a. With the redo log mechanism, there are two cache-line flushing (one for the log record and the other for tail pointer update), but only one barrier to persist them. The operation of applying the redo log to the modified $A$ also causes one cache-line flushing and one persistent barrier before the transaction is committed. 
%new log content copy to data also causes one cache line flushing and one store barrier before the transaction commit.%Assume there are also one append on object A in one transaction, we have two asynchronous cache write-back operations on the log, one $sfence$ barrier and one synchronous cache write-back operation on the data when we re-apply new value from log to original data place. 

%Figure~\ref{fig:undo_redo}.b shows the pseudo code of the redo log mechanism with a same example as undo log. With redo log, there are two cache-line flushing for log record and tail pointer update but only one barrier to persist them. The operation of new log content copy to data also causes one cache line flushing and one store barrier before the transaction commit.%Assume there are also one append on object A in one transaction, we have two asynchronous cache write-back operations on the log, one $sfence$ barrier and one synchronous cache write-back operation on the data when we re-apply new value from log to original data place. 

%The redo log reduces the ordering constraints on writes to persistent memory (avoid the synchronous cache write-back) but incurs an additional overhead for all the read operations in a transaction since each read operation has to consult the log for the latest value. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Copy-on-Write-based Persistent Transactions}
%\textcolor{blue}{kai, finish this subsection. Use the last subsection as an example.}


